Grounded Text-to-Image Synthesis with Attention Refocusing

Driven by the scalable diffusion models trained on large-scale datasets, text-to-image synthesis methods have shown compelling results. However, these models still fail to precisely follow the text prompt involving multiple objects, attributes, or spatial compositions. In this paper, we reveal the potential causes in the diffusion model's cross-attention and self-attention layers. We propose two novel losses to refocus attention maps according to a given spatial layout during sampling. Creating the layouts manually requires additional effort and can be tedious. Therefore, we explore using large language models (LLM) to produce these layouts for our method. We conduct extensive experiments on the DrawBench, HRS, and TIFA benchmarks to evaluate our proposed method. We show that our proposed attention refocusing effectively improves the controllability of existing approaches.

==> figures/ablation.tex <==
Using in-context learning vs. not...

Different Langauge Models

Different intermediate representations

==> sections/8_figures.tex <==


% MultiDiffusion~\cite{bar2023multidiffusion}  & \hspace{-0.2cm}Layout-guidance~\cite{chen2023training} & GLIGEN ~\cite{li2023gligen}

% \begin{figure*}[h]
%     \vspace{-0.5em}
%      \begin{subfigure}[t]{0.02\textwidth}
%         % \vspace{-8.6cm}
%         % \rotatebox[origin=c]{90}{
%         %     $\overbrace{\hspace{1.9cm}}_{\substack{\vspace{-6.8mm}\\\colorbox{white}{~~Ours~~}}}$
%         %     $\overbrace{\hspace{2.cm}}_{\substack{\vspace{-7.0mm}\\\colorbox{white}{~~GLIGEN~\cite{li2023gligen}~~}}}$
%         %     $\overbrace{\hspace{2.cm}}_{\substack{\vspace{-7.0mm}\\\colorbox{white}{~~MD~\cite{bar2023multidiffusion} ~~}}}$
%         %     $\overbrace{\hspace{2cm}}_{\substack{\vspace{-5.0mm}\\\colorbox{white}{~~LG~\cite{chen2023training}~~}}}$            
%         % }

%         \vspace{-16.8cm}
%         \rotatebox[origin=c]{90}{
%             $\overbrace{\hspace{4cm}}_{\substack{\vspace{-6.8mm}\\\colorbox{white}{~~GLIGEN+ Ours~~}}}$
%             $\overbrace{\hspace{4.cm}}_{\substack{\vspace{-7.0mm}\\\colorbox{white}{~~GLIGEN~\cite{li2023gligen}~~}}}$
%             $\overbrace{\hspace{4. cm}}_{\substack{\vspace{-7.mm}\\\colorbox{white}{~~MultiDiffusion~\cite{bar2023multidiffusion} ~~}}}$
%             $\overbrace{\hspace{4.3cm}}_{\substack{\vspace{-7.0mm}\\\colorbox{white}{~~Layout-guidance~\cite{chen2023training}~~}}}$            
%         }
        
%     \end{subfigure}
%     \begin{subfigure}[b]{0.97\textwidth}
%         \centering
%         \includegraphics[width=1.\textwidth]{figures/compare_4models_v2.pdf}
%         % \includegraphics[width=1.\textwidth]{figures/compare_4model.pdf}
%         \vskip -0.1cm
%         % \tabulinesep=-3mm
       
%     \end{subfigure}
%     % \vspace{-0.2cm}
%     \caption{
%     \tb{Visual comparisons on HRS benchmark.}
%     Here we apply our attention-based guidance on grouned text-to-image models.
%     All methods take the same grounded texts as inputs.
%     The results show the capability of our method in synthesizing novel spatial compositions and attributes.
%     % (MD: MUltiDiffusion, LG: layout-guidance, ours: GLIGEN + our losses).
%     % The qualitative results produced by ours and baselines. From left to right: Stable Diffusion, Attend-and-excite, text prompt, boxes, MultiDiffusion, layout-guidance, ours.
%     % While Stable Diffusion and Attend-and-excite use text as inputs, MultiDiffusion, layout-guidance, GLIGEN, and ours take text and layout as input. 
%     }
%     \label{fig:compare_basselines}
% \end{figure*}





==> sections/sup_application.tex <==
\section{Additional applications}
\subsection{Instructing text-to-image by chatGPT}
\label{sec:instruct}

We also propose a novel capability enabled by our framework, where users can utilize chatGPT to instruct text-to-image. In other words, after generating the initial layout and image, we instruct chatGPT to modify the layout, leading to an updated image. This iterative capability allows users to synthesize desired images through consecutive adjustments. As shown in ~\Fref{fig:instruct}, a user wants to generate an appealing image of "a hot air balloon flying over a field of four giant marshmallows". At first, the generated layout is not satisfying, so the user asks chatGPT to shift the balloon layout to the right and then adds the sun to its left. Such language-based refinement ability is difficult for traditional text-to-image models to offer.

\subsection{Video generation}


==> sections/sup_grounded_implementation.tex <==
\section{Implementation of grounded text-to-image models}
\label{sec:appendix}
\subsection{Data set and metrices}
\label{sec:adding_set_up}
\myparagraph{Dataset}

\tb{The HRS dataset} contains various prompts divided into three main categories: 1) accuracy, 2) robustness, and 3) generalization. 
Our method focuses on \emph{accuracy improvement}, including four main categories: \emph{spatial relationship, color, size, and counting}.
Each prompt in the dataset is tagged with the object's name and corresponding labels intended for evaluation. 
For example, in spatial relationships, the labels include objects and their relative positions, such as ``on the left'' or ``on the right''. 
The prompts for each category counting/spatial/size/color are $3,000/1,002/501/501$. 
Depending on the number of objects and their relationship, we label the difficulty level of each prompt as easy, medium, and hard with roughly the same amount. 

\tb{The DrawBench dataset} consists of 39 prompts about \emph{Counting} and \emph{Positional (or spatial relationship)}. 
Since there are no labels for this benchmark, we manually create the label for each prompt based on the number of objects mentioned and their relationships. 

\tb{The TIFA benchmark} contains $4,000$ prompts in various categories (counting, spatial, food, locations, etc...) and the questions for each prompt, along with their answers.


\myparagraph{Evaluation metrics.}
We use metrics in the HRS to compute the accuracy of individual categories. 
For counting, the precision, recall, and F1 scores are used to measure text-to-image models.
False positive samples happen when the number of generated objects is smaller than the ground truths. 
In contrast, the false negative objects are counted for the missing objects in the synthesized images. 
For other categories, we use accuracy as the evaluation metric. 
Depending on the category, the image is counted as a correct prediction when all detected objects are correct for spatial relationships, color, or size.

For the TIFA benchmark, we assess the alignment between the generated images and input texts using TIFA score. 
This metric is calculated based on a question-answering model, which uses generated images as input and outputs an answer for the specific question in the dataset. 
Then, the predicted answer is compared with the corresponding ground truth.  

\subsection{Implementation details of CAR and SAR losses }
\label{sec:adding_set_up}
We apply Cross-Attention Refocusing and Self-Attention Refocusing losses on the attention maps of resolution $16\times 16$. 
All images are generated with $50$ steps of denoising. 
We discuss setting details for optimization during denoising steps, referring to Eq.~\supref{(7)} 
In terms of $\tau$, in the very early steps ($t=0$ or $t=1$), the cross and self-attention maps are unclear yet begin to form the layout. 
So, we just set the iteration step $\tau=2$. 
Then, to make the layout clearer ($t \in \{2,3,4\}$), $\tau$ is increased to 6 steps, which helps refine the layout if tokens do not attend to the corresponding boxes or are in the wrong boxes. 
We also apply early stopping to reduce inference time and ensure the quality of generated images. 
We observe that applying optimization in later steps can lead to quality degradation. Therefore, after the first ten denoising steps, we only update the latent when the tokens do not align with the corresponding boxes or with incorrect ones.
The initial step size $\alpha$ is set to $4$ in the first five steps, then decreases to $3$. The detail of the algorithm can be seen in Algorithm ~\ref{algorithm}

In this paper, we use a Gaussian kernel with filter size 3 × 3 and a $\sigma$ value of 0.5 for standard deviation

In terms of four baselines, layout-to-image models: layout-guidance, MultiDiffusion, Attend-and-Excite, GLIGEN,  they are set default in their original papers.

\begin{algorithm}
\DontPrintSemicolon
\caption{Denoising step with Attention-Refocusing}

\KwData{A text prompt $P$, a set of token indices $I$, each token associates with a set of bounding box $B_{i}$ , a timestep $t$, a set of iterations for refinement \{$t_1,\dots,t_k$\}, the threshold $T$, and a trained Stable Diffusion model SD.}
\KwResult{latent $x_{t-1}$ for the next timestep}

$A^t, S^t \leftarrow SD(z, P, t)$\;
$A^t \leftarrow \text{Softmax}(A_t - \text{sot}())$\;
\For {$i \in I$}{
    
    $A_i^t \leftarrow A_{t[:,:, i]}$\;
    $A_i^t \leftarrow \text{Gaussian}(A_i^t)$\;
    $L_i^{t,FG} \leftarrow 1 - \max(A_i^t \cdot \text{Mask}(B_i))$\;
    $L_i^{t,BG} \leftarrow \max(A_i^t \cdot (1- \text{Mask}(B_i)))$\;
    $L_{i,CAR} \leftarrow L_i^{FG} + L_i^{BG}$\;
    \For {$p \in \text{Mask}(B_i)$}{
       $L_p = \sum_{p \in B_i}(\text{Average}(S_p^t \cdot (1 - \text{Mask}(B_i))$ 
    }
    $L_{i,SAR} = \sum_{p}(L_p)$
}
$L_{CAR} \leftarrow \sum_i(L_{i, CAR})$\;
$L_{SAR} \leftarrow \sum_i(L_{i, SAR})$
% \For { $(b,m) \in  (B,M)$}{
%     \For {$p \in b$}{
%         $L_p \leftarrow \textbf{average}(S_p^t * m)$
%     }
%     $L_b \leftarrow \sum_p(L_p)$
% }

% $L_{SAR} \leftarrow \sum_b (L_b)$\;
$L \leftarrow L_{CAR} + L_{SAR}$\;
$\hat{x}_t \leftarrow x_t - \alpha_t \nabla_{x_t} L$\;
\If{$t \in \{t_1, \dots, t_k\}$}{
    \If{$L > 1 - T$}{
        $x_t \leftarrow \hat{x}_t$\;
        Go to Step 1\;
    }
}
$x_{t-1} \leftarrow SD(\hat{x}_t, P, t)$\;
\Return $x_{t-1}$\;
\label{algorithm}
\end{algorithm}

\subsection{Applying CAR loss for segmentation mask}
\label{sec:adding_seg}
We also adapt the CAR loss to other layout modalities like depth maps, segmentation masks, and edge maps. 
Specifically, we always use the converted segmentation masks $M_i$ associated with token $i$-th to apply our method. 
Since the segmentation provides a precise object boundary in contrast to the bounding box, we optimize the attention over the entire foreground by taking the average instead of the maximum. 
The foreground loss for segmentation masks is: 
\begin{equation}
  \mathcal{L}_{FG} = \frac{1}{q} \sum_{i \in I}  \frac{\sum(1 - (A_i^t \cdot  M_i))}{\sum M_i}
\end{equation}
Similarly, the background loss for segmentation maps is:
\begin{equation}
  \mathcal{L}_{BG} = \frac{1}{q} \sum_{i \in I} \frac{\sum A_i^t \cdot (1- M_i)}{\sum (1 - M_i)}
\end{equation}
The $L_{SAR}$ is calculated using the formulation for bounding box presented in the main paper.
The results of applying our losses to ControlNet are shown on our website (open the file index.html)
% \begin{figure*}[t]

%     \centering
%     \includegraphics[width=1\textwidth]{figures/controlnet_big.pdf}
  
%       \begin{tabu} to 1.\textwidth {X[2cm,c]X[1.9cm,c]X[1.9cm,c]X[1.9cm,c]X[1.9cm,c]X[1.9cm,c]}
%         Input & ControlNet ~\cite{zhang2023adding}&ControlNet + Ours & Input & ControlNet ~\cite{zhang2023adding} & ControlNet + Ours\\
%         % \begin{tabu} to 0.5\textwidth {X[2cm,c]X[1.9cm,c]X[1.9cm,c]}
%         % Input & ControlNet ~\cite{zhang2023adding}&ControlNet + Ours \\
       
%         \end{tabu}
    
% % \hfill Stable Diffusion~\cite{bakr2023hrs} \vspace{2cm} 
% \caption{
% \tb{ControlNet with attention-based guidance.}
% % The input of ControlNet is a above image of input. With an extra segmentation map(in under images of input)
% In the input columns, upper representations are inputs of ControlNet, and lower ones are segmentation masks used for our losses. Applying our losses can refine the attribute blending of ControlNet.}
% \label{fig:controlnet_append}
% \end{figure*}



==> sections/sup_instruct.tex <==
\section{Additional applications}
\subsection{Instructing text-to-image by chatGPT}
\label{sec:instruct}

We also propose a novel capability enabled by our framework, where users can utilize chatGPT to instruct text-to-image. 
In other words, after generating the initial layout and image, we instruct chatGPT to modify the layout, leading to an updated image. 
This iterative capability allows users to synthesize desired images through consecutive adjustments. 
As shown in ~\Fref{fig:instruct}, a user wants to generate an appealing image of "a hot air balloon flying over a field of four giant marshmallows". At first, the generated layout was not satisfying, so the user asked chatGPT to shift the balloon layout to the right and then add the sun to its left. Such language-based refinement ability is difficult for traditional text-to-image models to offer.
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/songwei_ari_2.pdf}
    \caption{ Instruct text-to-image by instructing chatGPT.}
    \label{fig:instruct}
    \vspace{-0.4cm}
\end{figure}

\begin{table}[t!]
    \centering
    \caption{Comparison of Attention-refocusing and Boxdiff in the F1 score in counting and  accuracy(\%) in all spatial, size, and color categories in the HRS benchmark.}
    \label{tab:boxdiff}
    \footnotesize{
    \tabulinesep=0pt
    \begin{tabu} to 1.\columnwidth {@{}X[2.6, l]X[1.3,c]X[1.3,c]X[1.3,c]X[1.3,c]@{}}
        \toprule
        \multirow{2}{*}{\textbf{Method}} &\textbf{Counting}&\multicolumn{3}{c}{ \textbf{Compositions}}\\
         \cmidrule(r){2-2} \cmidrule(r){3-5}
         \footnotesize &\hspace{-0.2cm} F1~$\uparrow$ & \hspace{-0.2cm}Spatial~$\uparrow$ & \hspace{-0.45cm}Size~$\uparrow$& \hspace{-0.3cm}Color~$\uparrow$ \\
        \midrule
        GLIGEN + ours & \hspace{-0.38cm}\textbf{67.54} & \hspace{-0.5cm}\textbf{40.22} & \hspace{-0.5cm}27.74 & \hspace{-0.6cm} \textbf{26.32} \\
        \midrule
        GLIGEN + Boxdiff  & \hspace{-0.38cm} 67.02 &\hspace{-0.5cm} 33.93 & \hspace{-0.5cm}  \textbf{28.54 }&\hspace{-0.6cm} 22.50 \\
        % LLM-grouned SD & & 48.40&\\
        \bottomrule
    \end{tabu}
    }
\end{table}

==> sections/sup_layout.tex <==
\section{Layout generation}
\subsection{Full prompt for GPT-4}
\label{sec:gpt-4}
Our full prompt mainly includes the three components:\\
\textbf{Instruction} specifies the task and defines the output format. This instruction helps GPT-4 perform better in layout generation tasks.\\
\textbf{In-context exemplars} are used further to enhance the model's capacity for the task. 
We supplement user prompts with multiple examples for the best context understanding. This also helps the model output the desired form of bounding boxes and their corresponding labels. \\
\textbf{User prompt} is appended to the instruction and the supporting examples. Then, the model completes the chat conversation from the user prompt and returns the layout in the defined form.


Once the user provides a prompt (user prompt), it will be added to the defined and fixed text to create a full prompt shown in ~\Tref{tab:chatgpt}. Then, the GPT-4 API completes the chat and returns the box coordinates of the corresponding objects.

The comparison of our two-stage text-to-image models with single-stage one ( Stable diffusion) and several appealing results generated from our framework can be found on our website (open the file index.html).

\subsection{Comparison of four language models}
\myparagraph{Metrices for large language models evaluation}
We evaluate large language models in three metrics:
\begin{itemize}

\item Format: whether or not the model returns the correct format of grounded information, including four coordinates for each box and its label.

\item Validness: all generated boxes are satisfied with the size and box constraints, eg. the coordinate box is $\{x_1,y_1,x_2,y_2\}$ then $512 \ge x_1, x_2, y_1, y_2 \geq 0$,  $x_1 \leq x_2 $ and $y_1 \leq y_2$,

\item Correctness: the generated grounding information should follow the text prompts. For example, in terms of counting, the quantity of generated boxes should match the number of objects mentioned in the input prompt. In spatial and size categories, we asses the relations and relative size of generated boxes. Meanwhile, in color, we verify if the correct colors are returned for each object in the grounding text.
\end{itemize}

\myparagraph{The comparison of four language models} The results are shown in ~\Fref{fig:llama_gpt}. GPT-4 is capable of reasoning implicit object relationships. For instance, in the first prompt, a squirrel with a leather racket, GPT-4 can place the leather racket box centrally within the squirrel box, unlike GPT-3, Llama 2, and Llama1, which miss the spatial composition. However, the GPT-4 still struggles with some extremely hard prompts. For prompts with too many objects, GPT-4 can generate the correct number of objects but with small boxes.
\begin{table*}
\centering
    \caption{The full prompt for gpt4 api.  }
    \label{tab:chatgpt}
    \tabulinesep=4pt
    \begin{tabu} to 1.\textwidth {@{}X[1.9,l]X[9,l]@{}}
    \toprule
    \textbf{Role} & \textbf{Content} \\
    \midrule
      \textbf{Instruction}& System:{ "You are ChatGPT-4, a large language model trained by OpenAI. Your goal is to assist users by providing helpful and relevant information. In this context, you are expected to generate specific coordinate box locations for objects in a description, considering their relative sizes and positions and the number of objects. The box coordinates should be in the order ( left, top, right, bottom). The size of the image is 512*512."}\\
    \midrule
     \multirow{4}{*}{\textbf{In-context examples}} & User: {"Provide box coordinates for an image with a cat in the middle of a car and a chair. Make the size of the boxes as big as possible."}\\
     & Assistant: "cat: (245, 176, 345, 336); car: (10, 128, 230, 384);  chair: (353, 224, 498, 350)" \\
    % & User : "The sizes of objects do not reflect the object's relative sizes. The car's box size is similar chair's box size, and the cat's box size is quite similar to the car and chair. the car should be larger than the chair, and the chair should be larger than the cat."\\
    %  &  Assistant: "Apologies for the mistake. Here are the corrected coordinates: cat: (245, 176, 345, 336); car: (10, 128, 230, 384);  chair: (353, 224, 498, 350)" \\
    & User : "Provide box coordinates for an image with three cats on the field."\\
    
     &Assistant: "cat: (51, 82, 399, 279);cat: (288, 128, 472, 299); cat: (27, 355, 418, 494)"\\
    \midrule
    \textbf{User prompt} & User : "Provide the Provide box coordinates for an image with" + [user prompt]\\
    \bottomrule
    \end{tabu}
\end{table*}
% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=1.\textwidth]{figures/AE_SD_GLIGEN.pdf}
%     \begin{tabu} to 1.\textwidth {X[1.2,c]X[1.2,c]X[0.6,c]X[1.2,c]}
%         % \hline
%         \rule{0pt}{-1cm} Stable Diffusion & Attend-and-Excite & Layout from GPT-4  &  Ours
%         % \hline
%     \end{tabu}
    
%     \caption{Comparison current text-to-image models (Stable diffusion and Attend-and-excite) and two-stage pipeline (layout generated from GPT-4) }
% \end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=1.\textwidth]{figures/llama_gpt_small.pdf}
    \begin{tabu} to 1.\textwidth {X[1.2,c]X[1.2,c]X[1.2,c]X[1.2,c]}
        % \hline
        \rule{0pt}{-1cm} Llama 1  &LLama 2 & GPT-3 ~ &  GPT-4 
        
    \end{tabu}
    
    \caption{Comparison generated layouts from Llama 1, Llama 2, GPT-3, GPT-4 }
    
    \label{fig:llama_gpt}
\end{figure*}
    

==> sections/sup_quantitative.tex <==
\section{Additional quantitative results}
\label{sec:additional_quant}
The ~\Tref{tab:drawbench} shows results of our methods in the drawbench . Our proposed losses demonstrate a comparable performance boost to HRS. 
By integrating our losses, we compare favorably or comparatively against baselines in the counting procedure. 
Moreover, our losses substantially improve the accuracy of the spatial category.  

We also compare attention-refocusing loss with Boxdiff in ~\Tref{tab:boxdiff}. It can be seen that Attention-refocusing losses outperform Boxdiff in counting, spatial and color categories, especially in spatial composition, our method surpasses Boxdiff around 7\%. 

We compare the time inference of our losses and other free-training methods in  ~\Tref{tab:time}. Our losses are compatible with Attend-and-excite  , even more effective than Layout-guidance  in speed.
\begin{table}[t]
    \centering
    \caption{Quantitative evaluation on the DrawBench benchmark.}
    \label{tab:drawbench}
    \footnotesize{
    \tabulinesep=0pt
    \begin{tabu} to 1.\columnwidth {@{}X[1.7, l]X[0.7,c]X[1.3,c]X[1.1,c]X[1.3,c]X[1.2,c]@{}}
        \toprule
        \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\shortstack[c]{\textbf{CAR} \\ \& \textbf{SAR}}} &\multicolumn{3}{c}{\textbf{Counting}} &\hspace{-0.3cm} \textbf{Spatial}\\
         \cmidrule(r){3-5} \cmidrule(r){6-6}
         \footnotesize & & Precision~$\uparrow$ & \hspace{-0.2cm}Recall~$\uparrow$ & \hspace{-0.45cm}F1~$\uparrow$& \hspace{-0.3cm}Accuracy~$\uparrow$ \\
        \midrule
        \multirow{2}{*}{\shortstack[l]{Stable Diffusion \\}} & \xmark &  \hspace{-0.4cm}73.32   & \hspace{-0.35cm}70.00  &  \hspace{-0.45cm}71.55  &  \hspace{-0.4cm}12.50 \\
        & \cmark & 78.53~\goodi{5.2}   & 73.63~\goodi{3.6}  &  75.81~\goodi{4.3} &  43.50~\goodi{31.0} \\
        \midrule
        \multirow{2}{*}{\shortstack[l]{Attend-and-excite \\ }} & \xmark &  \hspace{-0.4cm}77.64   & \hspace{-0.35cm}74.85  &  \hspace{-0.45cm}76.20 &  \hspace{-0.4cm}20.50 \\
        & \cmark & 74.06~\badi{3.6}  & 77.58~\goodi{2.7}  &  75.66~\badi{0.5} &  38.00~\goodi{18.0} \\
        \midrule
        % Layout predictor &     &   &   &    \\
        \multirow{2}{*}{\shortstack[l]{Layout-guidance \\}} & \xmark & \hspace{-0.4cm}79.15    & \hspace{-0.35cm}70.61  &  \hspace{-0.45cm}74.48 & \hspace{-0.4cm}36.50   \\
        & \cmark & 78.45~\badi{0.7} &  75.45~\goodi{4.8} & 76.82~\goodi{2.3}  &52.50~\goodi{16.0}\\
        \midrule
        \multirow{2}{*}{\shortstack[l]{MultiDiffusion }} & \xmark & \hspace{-0.4cm}75.37    &  \hspace{-0.35cm}65.61 & \hspace{-0.45cm}69.90  &  \hspace{-0.4cm}38.00  \\
        &\cmark & 84.30~\goodi{8.9} & 68.03~\goodi{2.4} & 75.20~\goodi{5.3} & 54.50~\goodi{16.5} \\
        \midrule
        \multirow{2}{*}{\shortstack[l]{GLIGEN \\ }} & \xmark & \hspace{-0.4cm}81.66 &  \hspace{-0.35cm}80.89 &  \hspace{-0.45cm}81.18 & \hspace{-0.4cm}48.00   \\
        & \cmark & 90.28~\goodi{8.6} & 86.21~\goodi{5.3} & 88.16~\goodi{7.0} & 64.00~\goodi{16.0}\\
        \bottomrule
    \end{tabu}}
    \vspace{-1em}
\end{table}

\begin{table}[t!]
    \centering
    \caption{Our proposed losses improve the baselines in the HRS Counting benchmark.}
    \label{tab:counting_hrs}
    \small{
    \tabulinesep=0pt
    \begin{tabu} to 1.\columnwidth {@{}X[2.2, m]X[0.7,c]X[1.4,c]X[1.4,c]X[1.3,c]@{}}
        \toprule
        \vspace{-1em}\textbf{Method} & \shortstack[c]{\textbf{CAR} \\ \& \textbf{SAR}} & \vspace{-1.2em}\textbf{Precision~$\uparrow$} & \vspace{-1.2em}\hspace{-0.5cm}\textbf{Recall~$\uparrow$} & \vspace{-1.2em}\hspace{-0.5cm}\textbf{F1~$\uparrow$}\\
        \midrule
        \multirow{2}{*}{\shortstack[l]{Stable Diffusion }} & \xmark & \hspace{-0.6cm}71.86 & \hspace{-0.6cm}52.19 & \hspace{-0.58cm}58.31 \\
        & \cmark & 81.56~\good{9.7}& 51.19~\bad{1.0} & 60.62~\good{2.3} \\
        \midrule
        \multirow{2}{*}{\shortstack[l]{Attend-and-excite }} & \xmark &  \hspace{-0.6cm}73.10 & \hspace{-0.6cm}54.79 & \hspace{-0.58cm}60.47 \\
        & \cmark & 75.94~\good{2.8} & 56.31~\good{1.5} & 62.71~\good{2.2} \\
        \midrule
        % Layout predictor &     &   &   &    \\
        \multirow{2}{*}{\shortstack[l]{Layout-guidance }} & \xmark & \hspace{-0.6cm}80.60 & \hspace{-0.6cm}45.83 & \hspace{-0.58cm}56.22   \\
        & \cmark &78.15~\bad{2.5}& 55.65~\good{9.8} & 63.01~\good{6.8} \\
        \midrule
        \multirow{2}{*}{\shortstack[l]{MultiDiffusion  }} & \xmark & \hspace{-0.6cm}78.96 & \hspace{-0.6cm}45.18 & \hspace{-0.58cm}55.18  \\
        &\cmark & 83.26~\good{4.3}& 45.71~\good{0.5} & 57.37~\good{2.2} \\
        \midrule
        % \multirow{2}{*}{\shortstack[l]{GLIGEN  }} & \xmark & \hspace{-0.6cm}80.04 & \hspace{-0.6cm}60.67 & \hspace{-0.58cm}68.28   \\
        % & \cmark & 87.20~\good{7.2}&62.03~\good{1.4} & 71.83~\good{3.6} \\
        \multirow{2}{*}{\shortstack[l]{GLIGEN  }} & \xmark & \hspace{-0.6cm}78.81 & \hspace{-0.6cm}59.44 & \hspace{-0.58cm}66.58  \\
        % & \cmark & 81.12~\good{7.2}&59.70~\good{1.4} & 67.83~\good{3.6} \\
        & \cmark & 81.25~\good{2.4}&59.39~\badi{-0.1} & 67.54~\good{0.7} \\
        % \midrule
        % Boxdiff  & - &\hspace{-0.6cm} 83.78 & \hspace{-0.6cm} 57.81 & \hspace{-0.58cm} 67.02\\
        % \midrule
        % LLM-grounded SD & &76.05 &62.60 & 67.51\\
        \bottomrule
    \end{tabu}}
\end{table}

\begin{table}[h]
    \centering
    \caption{Inference time of different methods (s$/$10 images). AE: Attend-and-Excite, MD: MultiDiffusion, LG: Layout-guidance, Ours: Attention-Refocusing}
    \label{tab:time}
    % \begin{tabular}{ccccccc}  
    \small{
    \tabulinesep=0pt
    \begin{tabu} to 1.\columnwidth {@{}X[0.6,c]X[0.6,c]X[0.6,c]X[1.1,c]X[0.6,c]X[1,c]X[1,c]@{}}
    \toprule
    \multicolumn{5}{c}{Stable Diffusion } & \multicolumn{2}{c}{GLIGEN}\\
    \cmidrule(r){1-5} \cmidrule(r){6-7}
    {SD} & {+AE} & {+MD} & {+LG} & {+Ours} & {GLIGEN} & {+Ours}\\ 
    % \cmidrule(r){1-5} \cmidrule(r){6-7}
    \midrule
    54.33 & 101.67 & 74.16 & 111.13 & 102.97 & 205.90 & 279.08\\ 
    \bottomrule
    \end{tabu}}
\end{table}



==> setup/graphicspath.tex <==
\graphicspath{{figures}, {examples}}



==> setup/macros.tex <==
% Macros - Jia-Bin Huang (jbhuang0604@gmail.com)

% \renewcommand{\baselinestretch}{0.991}       % for squeezing the draft into the page limit, do not use

% For the unsure command.
\usepackage{soul}
\usepackage{svg}

% \usepackage[accsupp]{axessibility} % Improves PDF readability for those with disabilities.

% \usepackage[final]{changes}

\newcommand{\tae}[1]{{\textcolor{blue}{Tae: #1}}}

% =========================================
% Useful macros
% =========================================

% Latin abbreviations
\def\etal{et~al.\_}			  % and others, and co-workers
\def\eg{e.g.,~}               % for example
\def\ie{i.e.,~}               % that is, in other words
\def\etc{etc}                 % and other things, and so forth
\def\cf{cf.~}                 % compare
\def\viz{viz.~}               % namely, precisely
\def\vs{vs.~}                 % against

\def\naive{na{\"i}ve\xspace}
\def\Naive{Na{\"i}ve\xspace}
\def\naively{na{\"i}vely\xspace}
\def\Naively{Na{\"i}vely\xspace}

% Math related
\DeclareMathOperator*{\argmin}{\arg\!\min} 
\DeclareMathOperator*{\argmax}{\arg\!\max}
\DeclareMathOperator*{\minimize}{minimize}

\DeclareMathAlphabet{\altmathcal}{OMS}{cmsy}{m}{n}
\DeclareMathAlphabet{\mathbfit}{OT1}{ptm}{bx}{it}

% Consistent margin adjustment for paragraphs, figures, and sections
\newlength\paramargin
\newlength\figmargin

\newlength\secmargin
\newlength\figcapmargin
\newlength\tabcapmargin

\setlength{\secmargin}{0.0mm}
\setlength{\paramargin}{0.0mm}
\setlength{\figmargin}{0.0mm}
\setlength{\figcapmargin}{-0mm}
\setlength{\tabcapmargin}{0.0mm}

\setlength{\fboxsep}{0pt}

\newcommand{\red}{\textcolor{red}}
\newcommand{\blue}{\textcolor{blue}}
\newcommand{\changed}{\textcolor{black}} 

% minipage
\newcommand{\mpage}[2]
{
\begin{minipage}{#1\linewidth}\centering
#2
\end{minipage}
}

\newcommand{\mfigure}[2]
{
\includegraphics[width=#1\linewidth]{#2}
}

% \newcommand{\myparagraph}[1]
% {
% \vspace{-2.5pt}\paragraph{#1}
% }

\newcommand{\myparagraph}[1]
{
\vspace{2mm}\noindent\textbf{#1}
}

% References for figures, tables, equations, and sections
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}} 
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\eqnref}[1]{\eqref{eq:#1}}
\newcommand{\thmref}[1]{Theorem~\ref{#1}}
\newcommand{\prgref}[1]{Program~\ref{#1}}
\newcommand{\algref}[1]{Algorithm~\ref{#1}}
\newcommand{\clmref}[1]{Claim~\ref{#1}}
\newcommand{\lemref}[1]{Lemma~\ref{#1}}
\newcommand{\ptyref}[1]{Property~\ref{#1}}

% Comments
\long\def\ignorethis#1{}
%\newcommand {\jiabin}[1]{{\color{cyan}\textbf{Jia-Bin: }#1}\normalfont}
%\newcommand {\junyan}[1]{{\color{red}\textbf{Jun-Yan: }#1}\normalfont}
\newcommand {\taesung}[1]{{\color{magenta}#1}\normalfont}
\newcommand {\songwei}[1]{{\color{blue}\textbf{Songwei: }#1}\normalfont}
\newcommand {\jiabin}[1]{}
\newcommand {\junyan}[1]{}
\newcommand {\quynh}[1]{{\color{cyan}#1}\normalfont}
%\newcommand {\taesung}[1]{}
% \newcommand {\songwei}[1]{}
\newcommand {\new}[1]{{\color{magenta}#1}\normalfont}

%\newcommand {\todo}{{\textbf{\color{red}[TO-DO]\_}}}
\def\newtext#1{\textcolor{blue}{#1}}
\def\modtext#1{\textcolor{red}{#1}}
%\newcommand{\note}[1]{{\it\color{blue} #1}}

\definecolor{methodred}{RGB}{248, 203, 173}
\definecolor{methodyellow}{RGB}{245, 220, 143}
\definecolor{methodgreen}{RGB}{197, 224, 180}
\definecolor{methodblue}{RGB}{180, 199, 231}

%\newcommand{\unsure}[1]{{\sethlcolor{yellow}\hl{#1}}}

\newcommand{\tb}[1]{\textbf{#1}}
\newcommand{\mb}[1]{\mathbf{#1}}

\newcommand{\jbox}[2]{
  \fbox{%
  	\begin{minipage}{#1}%
  		\hfill\vspace{#2}%
  	\end{minipage}%
  }}

\newcommand{\jblock}[2]{%
	\begin{minipage}[t]{#1}\vspace{0cm}\centering%
	#2%
	\end{minipage}%
}

% subfigures with automatic width
\newbox\jsavebox%
\newcommand{\jsubfig}[2]{%
	\sbox\jsavebox{#1}%
	\parbox[t]{\wd\jsavebox}{\centering\usebox\jsavebox\\#2}%
	}

%%%%%%%%%%%%%%%%	
%% \providelength command that will define a new length if not already defined, but
%% also checks whether the command passed as argument has been defined with
%% \newlength, in order to issue an error message if you try to use, say,
%% \providelength{\textit}
\makeatletter
\newcommand{\providelength}[1]{%
  \@ifundefined{\expandafter\@gobble\string#1}
   {% if #1 is undefined, do \newlength
    \typeout{\string\providelength: making new length \string#1}%
    \newlength{#1}%
   }
   {% else check whether #1 is actually a length
    \sdaau@checkforlength{#1}%
   }%
}

\newcommand{\sdaau@checkforlength}[1]{%
  % get the first five characters from \meaning#1
  \edef\sdaau@temp{\expandafter\sdaau@getfive\meaning#1TTTTT$}%
  % compare with the string "\skip"
  \ifx\sdaau@temp\sdaau@skipstring
    \typeout{\string\providelength: \string#1 already a length}%
  \else
    \@latex@error
      {\string#1 illegal in \string\providelength}
      {\string#1 is defined, but not with \string\newlength}%
  \fi
}
\def\sdaau@getfive#1#2#3#4#5#6${#1#2#3#4#5}
\edef\sdaau@skipstring{\string\skip}
\makeatother
%%%%%%%%%%%%%%%%%%%%%



==> setup/package.tex <==
% Fix "undefined control sequence \Everyshipout".
% \usepackage{everyshi}

% Figures
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{float}
\usepackage[justification=raggedright]{caption}	% makes captions ragged right - thanks to Bryce Lobdell
\usepackage{lscape}                                         % Useful for wide tables or figures.
\usepackage{wrapfig}
\usepackage{pgfplots}

% Algorithm
\usepackage[lined,ruled,linesnumbered]{algorithm2e}
\usepackage{animate} %% convert frames to video

% Table and list
\usepackage{booktabs}                   % Publication quality tables
\usepackage{multirow}

\usepackage{makecell}

\usepackage{paralist}
\usepackage{enumitem}
\setlist[enumerate]{itemsep=0mm}

% Math
% \usepackage{bm}                          % Make bold, italic math symbols
\usepackage{epsfig}                      % for figures
% \usepackage{times}
% \usepackage{mathptmx}
% \usepackage{mathtools}
% \usepackage{amsmath}   % Short math guide for LaTeX ftp://ftp.ams.org/pub/tex/doc/amsmath/short-math-guide.pdf

% Fonts
\usepackage{units}
\usepackage{color}

% Comments
% \usepackage{comment}

% Hyperlinks
\usepackage{url}  % Hyphenation of URLs.
%\usepackage[pagebackref=true,breaklinks=true,letterpaper=true,pagebackref=true,colorlinks,bookmarks=false]{hyperref}
% \usepackage[pagebackref,breaklinks,colorlinks,linkcolor=blue,citecolor=blue,urlcolor=blue,bookmarks=false]{hyperref}
% \usepackage{authblk}
% \usepackage{slashbox}
\usepackage{xspace}
% \usepackage[table]{xcolor}
\usepackage{grfext}
\PrependGraphicsExtensions*{.jpg,.png,.PNG}
\definecolor{firebrick}{HTML}{d48265}
\definecolor{lightfirebrick}{HTML}{c23531}
% \definecolor{firebrick}{rgb}{0.59, 0.1, 0.1}
% \definecolor{lightfirebrick}{rgb}{0.95, 0.33, 0.33}
\definecolor{grayblue}{HTML}{61a0a8}
\definecolor{lightgrayblue}{HTML}{2f4554}
\definecolor{turquoise}{rgb}{0., 0.4, 0.7}
\definecolor{lightturquoise}{rgb}{0.4, 0.8, 0.96}
\definecolor{goldyellow}{rgb}{0.964, 0.886, 0.4}
\definecolor{lightorange}{HTML}{C27000}
\definecolor{darkorange}{HTML}{D3A171}
% \definecolor{lightorange}{rgb}{1., 0.9, 0.3}
\definecolor{lightgreen}{HTML}{61a0a8}
\definecolor{darkgreen}{HTML}{749f83}


\usepackage{textcomp,gensymb}
% \usepackage{emoji}
\usepackage{tikz}
% \usepackage{times,color}
% \usepackage{parskip}
% %\usepackage{epsfig}
% %\usepackage{psfig}
% %\usepackage[pdftex]{graphicx} % new acmsiggraph.cls
% \usepackage{ifthen}
% %\usepackage[draft]{hyperref} % new acmsiggraph.cls
% \usepackage{float}
% \usepackage{alltt}
% \usepackage{mathenv}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{amsthm}
% %\usepackage{rotating}
% \usepackage{newlfont} % for Box
% %\usepackage{ulem}
% \usepackage{floatflt}
% \usepackage{wrapfig}
% \usepackage{fixltx2e}
% \usepackage{subfig} % for subfloat
% \usepackage{multirow}
% \usepackage{cleveref}
% \usepackage{algorithmic}
% \usepackage{CJKutf8} % Chinese


==> setup/slashbox.tex <==
% slashbox.sty by Koichi Yasuoka, May 27, 1993
%              minor modification by Toru Sato, May 31, 1993
\typeout{slashbox style by K.Yasuoka, May 1993.}%
\newbox\@slashboxa
\newbox\@slashboxb
\newbox\@slashboxc
\newcount\@slashboxwd
\newcount\@slashboxht
\newdimen\@slashsepl
\newdimen\@slashsepr
\def\slashbox{%
  \def\@slashboxpicture##1{%
    \put(0,0){\line(##1,1){\@slashboxwd}}%
    \put(0,\@slashboxht){\makebox(0,0)[tl]{\box\@slashboxa}}%
    \put(\@slashboxwd,0){\makebox(0,0)[br]{\box\@slashboxb}}%
  }%
  \@slashbox
}%
\def\backslashbox{%
  \def\@slashboxpicture##1{%
    \put(0,\@slashboxht){\line(##1,-1){\@slashboxwd}}%
    \put(0,0){\makebox(0,0)[bl]{\box\@slashboxa}}%
    \put(\@slashboxwd,\@slashboxht){\makebox(0,0)[tr]{\box\@slashboxb}}%
  }%
  \@slashbox
}%
\def\@slashbox{\@ifnextchar [{\@@slashbox}{\@@slashbox[0pt]}}
\def\@@slashbox[#1]{\@ifnextchar [{\@@@slashbox[#1]}{\@@@slashbox[#1][c]}}
\def\@@@slashbox[#1][#2]#3#4{%
% #1: width, #2: suppression of \tabcolsep on `l', `r', or `lr' side
% #3: left item, #4: right item
  \@slashsepl=\tabcolsep
  \@slashsepr=\tabcolsep
    \@tfor\@tempa :=#2\do{\expandafter\let
        \csname @slashsep\@tempa\endcsname=\z@}%
  \setbox\@slashboxa=\hbox{\strut\hskip\tabcolsep\shortstack[l]{#3}}%
  \setbox\@slashboxb=\hbox{\shortstack[r]{#4}\hskip\tabcolsep\strut}%
  \setbox\@slashboxa=\hbox{\raise\dp\@slashboxa\box\@slashboxa}%
  \setbox\@slashboxb=\hbox{\raise\dp\@slashboxb\box\@slashboxb}%
  \setbox\@slashboxc=\hbox{%
    \@tempdima=\wd\@slashboxa
    \advance\@tempdima by \wd\@slashboxb
    \advance\@tempdima by \@slashsepl
    \advance\@tempdima by \@slashsepr
    \@tempdimb=#1\relax%
    \ifdim\@tempdimb>\@tempdima \@tempdima=\@tempdimb\fi%
    \@tempdimb=\ht\@slashboxa
    \advance\@tempdimb by \dp\@slashboxa
    \advance\@tempdimb by \ht\@slashboxb
    \advance\@tempdimb by \dp\@slashboxb
    \@tempcnta=\@tempdima
    \@tempcntb=\@tempdimb
    \advance\@tempcnta by \@tempcntb
    \advance\@tempcnta by -1
    \divide\@tempcnta by \@tempcntb
    \ifnum\@tempcnta>6 \@tempcnta=6
      \@tempdimb=0.166666666\@tempdima
    \else
      \ifnum\@tempcnta<1 \@tempcnta=1\fi
      \@tempdima=\@tempdimb
      \multiply\@tempdima by \@tempcnta
    \fi%
    \advance\@tempdima by -\@slashsepl
    \advance\@tempdima by -\@slashsepr
    \@slashboxwd=\@tempdima
    \@slashboxht=\@tempdimb
    \@tempcntb=\@slashsepl
    \setlength{\unitlength}{1sp}%
    \begin{picture}(\@slashboxwd,\@slashboxht)(\@tempcntb,0)
    \advance\@tempdima by \@slashsepl
    \advance\@tempdima by \@slashsepr
    \@slashboxwd=\@tempdima
    \@slashboxpicture{\@tempcnta}
    \end{picture}%
  }%
  $\vcenter{\box\@slashboxc}$%
}%


==> setup/symbols.tex <==
% Define math symbols that appear in the texts

\def\xi{\mathbf{x}_i}
\def\yi{\mathbf{y}_i}

